Speak in the Scene: Diffusion-based Acoustic Scene Transfer toward Immersive Speech Generation

This paper introduces a novel task in generative speech processing, Acoustic Scene Transfer (AST), which aims to transfer acoustic scenes of speech signals to diverse environments. AST promises an immersive experience in speech perception by adapting the acoustic scene behind speech signals to desired environments. We propose AST-LDM for the AST task, which generates speech signals accompanied by the target acoustic scene of the reference prompt. Specifically, AST-LDM is a latent diffusion model conditioned by CLAP embeddings that describe target acoustic scenes in either audio or text modalities. The contributions of this paper include introducing the AST task and implementing its baseline model. For AST-LDM, we emphasize its core framework, which is to preserve the input speech and generate audio consistently with both the given speech and the target acoustic environment. Experiments, including objective and subjective tests, validate the feasibility and efficacy of our approach.

==> Experiments/graph_diffrent.tex <==
% proposed는 darkred로, 나머진 원하는 색으로 바꿔도 상관없음.
% 수정해야하는 건 \addplot안에 있는 값들
% 순서대로 -5, 0, 5, 10, 15, clean set에 대한 점수들을 적으면 됨.
% ymin, ymax로 plot에 표시할 y축 범위를 지정해야함.
% FAD ↓ & KL ↓ & CLAP ↑ & LSD ↓ & SSM
% C-C, C-E, E-C
\begin{figure}[t]
    \footnotesize
    \begin{minipage}[h]{0.48\columnwidth}
        \centering
        \begin{tikzpicture}
            \begin{axis}[
                width=1.2\columnwidth, height=0.8\columnwidth,
                scaled y ticks = false,
                scaled x ticks = false,
                xtick pos=left, ytick pos=left,
                ybar,
                bar width=5pt,
                enlargelimits=0.005,
                xmin=4, xmax=10,
                ymin=50,   ymax=100,
                xlabel={\bf FAD},
                x label style={at={(0.5,1.6)},font=\footnotesize},
                y label style={at={(0.14,0.5)},font=\footnotesize},
                xticklabels={C-C, C-E, E-C},
                xtick={5, 7,9},
                ytick={0, 20, 40, 50, 60, 70, 80, 90, 100},
                yticklabels={0, 20, 40, 50, 60, 70, 80, 90, 100},
                minor tick length=1ex,
                % major x tick style = {opacity=1},
                x tick label style={/pgf/number format/1000 sep=},
                ymajorgrids=true,
                xmajorgrids=true,
                grid style=dashed,
                % legend style={at={(0.81, -0.3)}, anchor=north, legend columns=-3},
                ]
                \addplot coordinates{
                (5, 75.8) (7,82.3) (9,87.6)}; % (C-C, C-E, E-C) for DiffRENT
                \addplot coordinates{
                (5, 74.1) (7,80.4) (9,86.1)}; % (C-C, C-E, E-C) for ASTLDM
                % \legend{DiffRENT, \textbf{ASTLDM}}
            \end{axis}
        \end{tikzpicture}
    \end{minipage}%
    \begin{minipage}[h]{0.48\columnwidth}
        \centering
        \begin{tikzpicture}
            \begin{axis}[
                width=1.2\columnwidth, height=0.8\columnwidth,
                scaled y ticks = false,
                scaled x ticks = false,
                xtick pos=left, ytick pos=left,
                ybar,
                bar width=5pt,
                enlargelimits=0.005,
                xmin=4, xmax=10,
                ymin=50,   ymax=100,
                xlabel={\bf KL},
                x label style={at={(0.5,1.6)},font=\footnotesize},
                y label style={at={(0.14,0.5)},font=\footnotesize},
                xticklabels={C-C, C-E, E-C},
                xtick={5, 7,9},
                ytick={0, 20, 40, 50, 60, 70, 80, 90, 100},
                yticklabels={0, 20, 40, 50, 60, 70, 80, 90, 100},
                minor tick length=1ex,
                % major x tick style = {opacity=1},
                x tick label style={/pgf/number format/1000 sep=},
                ymajorgrids=true,
                xmajorgrids=true,
                grid style=dashed,
                % legend style={at={(0.81, -0.3)}, anchor=north, legend columns=-3},
                ]
                \addplot coordinates{
                (5, 75.8) (7,82.3) (9,87.6)}; % (C-C, C-E, E-C) for DiffRENT
                \addplot coordinates{
                (5, 74.1) (7,80.4) (9,86.1)}; % (C-C, C-E, E-C) for ASTLDM
                % \legend{DiffRENT, \textbf{ASTLDM}}
            \end{axis}
        \end{tikzpicture}
    \end{minipage}%
    \vfill
    \begin{minipage}[t]{0.48\columnwidth}
        \centering
        \begin{tikzpicture}
            \begin{axis}[
                width=1.2\columnwidth, height=0.8\columnwidth,
                scaled y ticks = false,
                scaled x ticks = false,
                xtick pos=left, ytick pos=left,
                ybar,
                bar width=5pt,
                enlargelimits=0.005,
                xmin=4, xmax=10,
                ymin=50,   ymax=100,
                xlabel={\bf CLAP},
                x label style={at={(0.5,1.6)},font=\footnotesize},
                y label style={at={(0.14,0.5)},font=\footnotesize},
                xticklabels={C-C, C-E, E-C},
                xtick={5, 7,9},
                ytick={0, 20, 40, 50, 60, 70, 80, 90, 100},
                yticklabels={0, 20, 40, 50, 60, 70, 80, 90, 100},
                minor tick length=1ex,
                % major x tick style = {opacity=1},
                x tick label style={/pgf/number format/1000 sep=},
                ymajorgrids=true,
                xmajorgrids=true,
                grid style=dashed,
                % legend style={at={(0.81, -0.3)}, anchor=north, legend columns=-3},
                ]
                \addplot coordinates{
                (5, 75.8) (7,82.3) (9,87.6)}; % (C-C, C-E, E-C) for DiffRENT
                \addplot coordinates{
                (5, 74.1) (7,80.4) (9,86.1)}; % (C-C, C-E, E-C) for ASTLDM
                % \legend{DiffRENT, \textbf{ASTLDM}}
            \end{axis}
        \end{tikzpicture}
    \end{minipage}%        \vfill
    \begin{minipage}[b]{0.48\columnwidth}
        \centering
        \begin{tikzpicture}
            \begin{axis}[
                width=1.2\columnwidth, height=0.8\columnwidth,
                scaled y ticks = false,
                scaled x ticks = false,
                xtick pos=left, ytick pos=left,
                ybar,
                bar width=5pt,
                enlargelimits=0.005,
                xmin=4, xmax=10,
                ymin=50,   ymax=100,
                xlabel={\bf SSM},
                x label style={at={(0.5,1.6)},font=\footnotesize},
                y label style={at={(0.14,0.5)},font=\footnotesize},
                xticklabels={C-C, C-E, E-C},
                xtick={5, 7,9},
                ytick={0, 20, 40, 50, 60, 70, 80, 90, 100},
                yticklabels={0, 20, 40, 50, 60, 70, 80, 90, 100},
                minor tick length=1ex,
                % major x tick style = {opacity=1},
                x tick label style={/pgf/number format/1000 sep=},
                ymajorgrids=true,
                xmajorgrids=true,
                grid style=dashed,
                legend style={at={(0.5, -0.5)}, anchor=north, legend columns=2},
                ]
                \addplot coordinates{
                (5, 75.8) (7,82.3) (9,87.6)}; % (C-C, C-E, E-C) for DiffRENT
                \addplot coordinates{
                (5, 74.1) (7,80.4) (9,86.1)}; % (C-C, C-E, E-C) for ASTLDM
                % \legend{DiffRENT, \textbf{ASTLDM}}
            \end{axis}
        \end{tikzpicture}
    \end{minipage}
    \vspace{-5pt}
    \caption{Comparison of generation performance between DiffRENT ({\color{blue} Blue}) and \shortname~({\color{red} Red}) on the VCTK-DDS dataset.}
    \label{fig:diffrent}
\end{figure}


==> backup.tex <==
% abstract
% This paper presents a novel method for transferring the acoustic scene of speech signals onto different environments. 
% While speech recorded in a clean setting may accurately convey linguistic expression, listeners often perceive a perceptual discrepancy because real-world conversations rarely occur in an anechoic environment. 
% Our proposed approach aims to mitigate this disparity by transferring the acoustic scene of a reference speech onto the target speech, thereby providing a similar acoustic environment and enhancing the realism of the speech. 
% This method has potential applications for individuals recording speech or dubbing additional audio, allowing them to maintain continuity with previously recorded environments, as well as it contributes to making acoustic perception more realistic.
% Key contributions of this work include:
% 1) precise extraction of the reference acoustic scene from the reference speech audio and generation of new audio signals,
% 2) preservation of the speech content or speaking style of the input speech, and
% 3) emphasis on perceptual quality to generate realistic speech signals. 
% Our model builds upon the audio latent diffusion model, conditioning it on the acoustic embedding of both the reference speech and the input speech.
% Experimental results, including objective and subjective tests, validate the feasibility of our approach.



% % anechoic: <녹음실·방송실 등이> 울림[반향]이 없는 (from naver dict)
% This paper presents a novel method for transferring acoustic scenes of speech signal across diverse environments.
% While clean speech may accurately convey linguistic expression, listeners often perceive a perceptual discrepancy because real-world conversations rarely occur in an anechoic environment. 
% Our proposed approach aims to mitigate the disparity by transferring the target acoustic scene onto the input speech, providing a realistic perception. 
% Additionally, we extend this method to transfer acoustic scenes across various environments, not only from anechoic to environment. 
% Key contributions include precise extraction of reference acoustic scenes, preservation of input speech, and generation of audio carrying on given speech and target recording environment. 
% %environmental speech signals. 
% Our model builds upon the audio latent diffusion model, conditioning it on both reference and input speech embeddings. 
% Experimental results, including objective and subjective tests, validate the feasibility of our approach.

%% diffusion-based audio generation
% \pagebreak
% \section{Related Works}
% \subsection{Diffusion}



% %AudioLDM: clap conditioned text-to-audio
% %VoiceLDM: clap conditioned text-to-speech
% %DIFFRENT: acoustic scene transfer / diffusion model / overfitted to training set / realistic noise transferring / ambient noise / require training pairs
% %Proposed: acoustic scene transfer / latent diffusion model / clap


% % 2.1.1 Overview of diffusion
% Diffusion model is a state-of-the-art of generative model by adding Gaussian noise to the training data (forward process) and then estimating added noise from previous states to generate original data (reverse process).
% Nowadays diffusion model have achieved outstanding synthesis qualities for generation tasks across wide range of research fields. 
% An auxiliary classifier guidance is combined into diffusion model to achieve advanced synthesis quality of image~\cite{NEURIPS2021_49ad23d1}.
% Subsequently, classifier-free guidance constructs generative model by training a network with the both of unconditional and conditional score estimator, achieving a free of joint training with an additional classifier~\cite{ho2021classifier}. 
% To moderate the semantic contents in the generated samples, text description is conditioned to diffusion networks for guiding image generation~\cite{pmlr-v162-nichol22a, Gu_2022_CVPR}.

% % 2.1.2 Description of latent diffusion
% Although diffusion model shows off its high generative performances, progressively iterative generation process (reverse process) leads a slow inference speed. 
% Latent diffusion model (LDM)~\cite{Rombach_2022_CVPR} effectively resolves this limitation by implementing diffusion process in a diminished latent features obtained from a pre-trained Variational autoencoder (VAE)~\cite{DBLP:journals/corr/KingmaW13}.
% % 2.1.3 Examples of latent diffusion
% By leveraging multi-modal knowledge from CLIP ~\cite{pmlr-v139-radford21a}, which learns a united embedding space between image and text, text-to-image framework is proposed based on LDM~\cite{pmlr-v139-jia21b}. AR-LDM presents story visualization, generating a video that matches the text-based story~\cite{pan2024synthesizing}.

% %In audio generation task, TANGO utilized LDM for music generation conditioned on text descriptions~\cite{}. AudioLDM also focuses on text conditioned audio generation but it can cover expanded audio types by adopting contrastive language-audio pretraining (CLAP)~\cite{}.

% \subsection{Audio Generation}
% % 2.2.1 Token-based audio generation 
% In recent days, transformer-based audio generation can be divided roughly in two approaches. The one way is utilizing a sequence of discrete audio representations~\cite{}, relying on pre-trained neural compression frameworks such as Soundstream~\cite{9625818} or Encodec~\cite{}. Conditioned on text descriptions, AudioLM~\cite{10158503} combines semantic and acoustic tokens, which are extracted from w2v-bert and Soundstream respectively, in a hierarchical fashion to achieve long-term consistency and high quality audio synthesis. Focusing on music generation, MusicLM~\cite{} also adopts sequential discrete token estimations from text descriptions, relying on MuLan~\cite{}, a joint music-text model that is trained to project music and its corresponding text description to unified representation space.

% % 2.2.2 Diffusion-based audio generation 
% The other way of audio generation stream is leveraging an audio modeling power utilizing diffusion models. TANGO~\cite{} utilized LDM for music generation conditioned on text descriptions~\cite{}. AudioLDM also focuses on text conditioned audio generation but it can cover expanded audio types by adopting contrastive language-audio pretraining (CLAP)~\cite{}. Another case which utilizes CLAP for speech generation is VoiceLDM~\cite{}, which focuses of generating Text-to-Speech module conditioned with background noise from CLAP embedding. 

% %--Non diffusion--
% % AudioLM, MuLan, MusicLM, AudioGen
% %--Diffusion--
% % non-clap : DiffVoice, Prosody-TTS, DIffrent
% % with clap: AudioLDM, TANGO, DiffSound, VoiceLDM

% % 2.2.1 Overview of CLAP-based audio generation & description of AudioLDM
% % 2.2.2 VoiceLDM (random하게 text로부터 스피치 만들면 되기 때문에 상대적으로 쉬운 테스크임)
% % 2.2.3 
% %Some works focus on zero-shot editing using pre-trained diffusion models. Perhaps the simplest approach is SDEdit (Meng et al., 2021), which adds noise to the signal and then runs it through the reverse diffusion process with a different text prompt. SDEdit was recently used for audio (Liu et al., 2023a) as well as for piano-roll
% %music (Zhang et al., 2023a). However it suffers from a severe tradeoff between adherence to the text and adherence to the original signal. Another direction, which has become popular in the image domain, is to use inversion techniques that extract the diffusion noise vectors corresponding to the source signal. One method for doing so is DDIM inver- sion (Song et al., 2021; Dhariwal & Nichol, 2021). This method was found suboptimal for editing images on its own, and is therefore typically accompanied by intervention in the attention maps during the diffusion process (Hertz et al., 2022; Cao et al., 2023; Tumanyan et al., 2023). An- other approach is DDPM inversion (Huberman-Spiegelglas et al., 2023; Wu & De la Torre, 2023), which is concep- tually similar, but applies to the DDPM sampling scheme. Here we adopt the DDPM inversion method of Huberman- Spiegelglas et al. (2023), which has shown state-of-the-art results in the image domain.


% ASTLDM
% % \section{Proposed Method}
% \section{\shortname}

% % 3.0.0 Objective or proposed model
% Conditioned by content prompt (input speech) and reference prompt containing information of the target acoustic scene (audio or text), proposed diffusion-based framework aims to generate input speech recordings in the environments, which are described by the reference prompt.    
% % 3.0.1 Motivation of using Latent diffusion (VAE)
% Due to a long inference time of the vanilla diffusion model, we implement the diffusion process in a diminished dimension of latent embeddings encoded by a pre-trained VAE encoder. 
% % 3.0.2 Overall flow of proposed framework
% Figure 1 illustrates overall framework of proposed model. 
% Proposed framework is constructed with four modules, Eontent encoder~$F_C$, CLAP~$F_{CLAP}$, Latent generator~$F_L$, Variational autoencoder, and Hifi-gan Vocoder. 
% In detailed description, log mel-spectrograms of content prompt~$x_c$ are passing through the $F_C$ so that content embeddings~$e_c$ are generated from.   
% Reference prompts~$x_r$, formalized by audio or text, are passing through the CLAP module and then generate embeddings~$e_c$.
% And then, Latent embeddings~$y$ are generated from $F_L$ conditioned by $x_r$ and $e_c$.
% Mel-spectrograms are decoded from a VAE decoder and raw speech waveforms are generated using a Hifi-gan vocoder using estimated mel-spectrograms.
% In the following, we describe each component in detail.

% \subsection{Reference Prompt}
% % 3.2.1 Motivation of using CLAP
% For the shake of extracting acoustic scene information from reference prompts, we bring a pre-trained CLAP module which maps audio and corresponding text description into the sole united latent space.
% For this reason, only one modality is enough for obtaining CLAP embedding, thus we chose audio to obtain the descriptive acoustic condition from CLAP.
% % 3.2.2 Description about reference prompt 
% For input audio as reference prompts, speech samples recorded in the target environments are employed. 
% Since not only speech is contaminated by background noise, it could be reverberated by an indoor room impulse response.
% Considering mentioned immersive situation, we simulated noisy speech by combining clean speech with the room impulse response and diverse types of background noise.
% %Thus the latent diffusion is conditioned on clap embeddings from audio or text so that latent embeddings are generated from, which include target acoustic scene information.

% \subsection{Content Prompt}
% % 3.1.1 Description about content prompt 
% Content prompts~$x_c$ are input speech recordings that supplies speech-related information to the framework, such as linguistics and characteristics of speakers.
% We carefully consider total 4 types of content prompt as follows; speech only, speech contaminated with background noise, speech reverberated with room impulse response, speech reverberated with room impulse response and contaminated with background noise. 
% % 3.1.2 Description about content encoder 
% The goal of the content encoder $F_C$ is acquiring $e_c$ from $x_c$, which includes speaker and linguistic features only.
% To achieve the objective, the content encoder consists of two components, filter module~$C_f$ and content module~$C_c$.
% The $C_f$ estimates mask from given $x_c$ filtering out unnecessary information from given audio prompt using 2 of transformer encoder layers followed by sigmoid function.
% After multiplying $x_c$ with estimated mask, $e_c$ is obtained by passing through this filtered embeddings into the $C_c$, which is constructed with 2 of CNN blocks and 4 of transformer encoder layers in order.
% Both $C_f$ and $C_c$ utilized 256 hidden dimensions and 8 attention heads of transformer encoder layers.

% \subsection{Latent Diffusion}
% Given $x_r$ and $e_c$, which contains recording environments and speech-related features respectively, $F_L$ aims to generate latent features $y$, which finally decoded to the mel-spectrogram passing through the pre-trained VAE decoder.
% %The latent generator is composed of a pre-trained CLAP and U-net module.
% %The CLAP module utilizes $x_r$ as input and then generates 512 dimension of clap embeddings $e_{clap}$ which contain overall audio information of given mel-spectrograms.
% % (miseul): cross attention 말고 adding 하면 성능 떨어졌다는거 언급.
% The Unet backbone predicts the diffusion score conditioned on $e_{clap}$ and $e_c$, conditioned on concatenation with latent features and cross-attention to the bottleneck layer of U-net respectively.
% Starting from a random noise sampled from an Gaussian noise (mean=0, dev=1) $z_t$, the reverse diffusion process iteratively denoises $z_t$ for each time step t with the predicted diffusion score and predicts the initial audio prior $y$. 
% After estimated latent features $y$ are decoded back to the mel-spectrogram by the pre-trained VAE decoder, the pre-trained HiFi-GAN vocoder converts the mel-spectrogram into desired raw audio wavefrom.


% experimental settings


% \subsection{Dataset}
% % Description of datset
% To simulate clean speech distorted with background noise and reverberated in room scenario, we utilized publicly available dataset only for network training; 960 hours of Librispeech, AudioCaps, Balanced set in Audioset, VggSound, DNS-Challenge impulse response and 26 speakers in DDS dataset. 
% In AudioCaps, samples containing non-speech set only are elected.
% In DDS dataset, we put aside speaker p234, p241 and recording environment of 'livingroom1 in Uber' to compare the performance with model DIFFRENT~\cite{}.
% % Mixing method
% We constructed followed 4 types of prompt using clean speech, contaminated clean speech with noise, reverberated speech combined with background noise and just reverberated clean speech. 
% Since there are 4 of possible types for prompt, total 16 pairs of audio and content prompt can passing through the modules respectively.
% Specifically, clean speech from Librispeech is mixed with randomly chosen noise set from AudioCaps, balanced set in Audioset, or VggSound and convolved with impulse response set from DDS dataset.
% For DDS dataset, we didn't applied any distortion to samples.
% After generating both audio and context prompts, target mel-spectrograms are generated by mixing with clean speech from context prompt and background noise or presence of reverberation from audio prompt.
% Both length of audio and content prompt is segmented with 10 second, so if samples are shorter than 10 seconds, we padded zero into the speech signal to match 10 seconds. 

% \subsection{Training Strategy}
% % DCFG
% % optimizer, learning rate...
% % 데이터의 구성 (simulated & real)

% Since the network utilizes two conditions $x_r$ and $x_c$ for latent synthesis, we adopted dual-classifier free guidance as done in ~\cite{}.
% During network training, we randomly dropped $x_r$ and $x_c$ 0.1 and 0.1 respectively.
% Although $x_c$ is not a prompt of clean speech only, it includes plenty of speech-related information which are closely related to target latent features, so we increased drop ratio of $x_c$ compared to the one of $x_r$.
% The model is trained to predict the added noise by minimizing the distance between the added noise using mean-squared error.
% During training VAE, CLAP, and Hifi-gan vocoder are left in frozen so that only the gradient of content encoder, U-net backbone are jointly updated.

% \subsection{Implementation Details}
% % Hidden dim
% % Number of parameter...
% % STFT, mel bins.... specification

% experimental results
% % 5.1.1 Description of Objective metrics
% \paragraph{Objective metrics} 
% To check the similarity between reference prompt audio and synthesized audio, we measured Frechet Audio Distance (FAD)~\cite{}, Kullback-Leiber (KL) divergence~\cite{}, and CLAP score~\cite{}.
% Moreover, we adopted word error rate (WER) to evaluate speech intelligibility employing Whisper large-v2~\cite{}.
% Since there are pair dataset in DDS dataset, we calculated the log-spectral distance (LSD)~\cite{} and speaker similarity (SSM)~\cite{} between target speech and synthesized speech.

% % 5.1.2 Description of Subjective metrics
% \paragraph{Subjective metrics} We conducted listening test for 20 respondents to confirm overall quality (OQ) of generated samples and environment similarity (ES) between synthesized and ground-truth samples in DDS dataset.
% To check overall quality of samples, 5 MOS test requiring listeners to evaluate overall speech qualities scoring from 1 (bad) to 5 (excellent) in integer scale.
% For environment similarity measurements, subjects are asked to score from 1 (Totally different) to 5 (Exactly same) in integer scale after listening two samples.
% Since VoiceLDM only utilizes text as an content prompt, we gave corresponding text of target DDS samples as a contemt prompt of VoiceLDM.


% (miseul) 성능평가 scheme 
% Exp1: Text를 condition 받은 경우 성능 평가 (AudioLDM, VoiceLDM과의 비교실험 가능)
    % FAD, KL, CLAP, WER (voiceldm only)
    % Input 바꿔가며 clean / clean + noise / clean + reverb / clean + noise + reverb
    % clean + noise + reverb에 대해서 masking 안한 모델
% Exp2: Simulated dataset에 대한 실험
    % FAD / KL / CLAP / WER / SSM
    % CC / CE / EE
% Exp3: DIFRRENT와 비교실험 in DDS
    % DEMO 페이지에 잇는 샘플만 사용해서 평가할 것 (P234, 241)
    % FAD, KL, CLAP, LSD, SSM 
    % env-env / clean-env / env-clean 세가지 측정
% Exp4: Subjective test in DDS
    % Quality MOS / Environment similarity 
    % Target / VoiceLDM / DIFRRENT / Proposed

% (miseul): tgt enhance module도 같이 학습해서 ablation 진행. 뚝뚝끊김.
% 음성 생성시에 10개 샘플 중 clap embedding sim 제일 높은거로 선택
% 고민해볼 것
    % DIFFRENT는 structural similarity (SSIM)를 쟀던데, 이게 뭐지? 
    % PESQ, SiSPNR (DIFFRENT에서 잿음)와 같은 평가지표도 측정 필요한가?
    % Exp1: % clean + noise + reverb에 대해서 tgt clean mel loss 추가한 모델 ?
    
